Text and Patterns: For Effective Chain of Thought, It Takes Two to Tango

The past decade has witnessed dramatic gains in natural language processing and an unprecedented scaling of large language models. These developments have been accelerated by the advent of few-shot techniques such as chain of thought (CoT) prompting. Specifically, CoT pushes the performance of large language models in a few-shot setup by augmenting the prompts with intermediate steps. Despite impressive results across various tasks, the reasons behind their success have not been explored. This work uses counterfactual prompting to develop a deeper understanding of CoT-based few-shot prompting mechanisms in large language models. We first systematically identify and define the key components of a prompt: symbols, patterns, and text. Then, we devise and conduct an exhaustive set of experiments across four different tasks, by querying the model with counterfactual prompts where only one of these components is altered. Our experiments across three models (PaLM, GPT-3, and CODEX) reveal several surprising findings and brings into question the conventional wisdom around few-shot prompting. First, the presence of factual patterns in a prompt is practically immaterial to the success of CoT. Second, our results conclude that the primary role of intermediate steps may not be to facilitate learning how to solve a task. The intermediate steps are rather a beacon for the model to realize what symbols to replicate in the output to form a factual answer. Further, text imbues patterns with commonsense knowledge and meaning. Our empirical and qualitative analysis reveals that a symbiotic relationship between text and patterns explains the success of few-shot prompting: text helps extract commonsense from the question to help patterns, and patterns enforce task understanding and direct text generation.

==> tables/all_counterfactual_thoughts.tex <==
\begin{table}[!ht]
\small
\begin{tabular}{p{3cm}p{4cm}p{6cm}}
\toprule
\textbf{Prompt} & \textbf{Definition} & \textbf{Sample Thought} \\
\toprule
\direct  &  No thought is used. This is the baseline few-shot setup. & ---  \\ \midrule
\pcot &  Identical thoughts as \citet{wei2022chain} are used. & Shawn started with 5 toys. If he got 2 toys each from his mom and dad, then that is 4 more toys. 5 + 4 = 9.\\\toprule
\multicolumn{3}{c}{$\LHD\,$\bm{\symbhl{Symbols}}$\,\RHD$}\\\toprule
\psymbabs & All the symbols are replaced with abstract placeholders. & Shawn started with \symbhl{\bm{$\alpha$}} toys. If he got \symbhl{\bm{$\beta$}} toys each from his mom and dad, then that is \symbhl{\bm{$\lambda$}} more toys. \symbhl{\bm{$\alpha$}} + \symbhl{\bm{$\lambda$}} = \symbhl{\bm{$\pi$}}. \\  \midrule
\psymbood  & Symbols are replaced with out-of-distribution values. &  Shawn started with \symbhl{5.5} toys. If he got \symbhl{2.5} toys each from his mom and dad, then that is 5 more toys. \symbhl{5.5} + \symbhl{5} = \symbhl{10.5}. \\  \midrule
\multicolumn{3}{c}{$\LHD\,$\bm{\pathl{Patterns}}$\,\RHD$}\\\toprule
\pwrongpat & Patterns are changed to reflect incorrect final answer. & Shawn started with 5 toys. If he got 2 toys each from his mom and dad, then that is 4 more toys. 5 \pathl{+} 4 \pathl{=} 7. \\  \midrule
\pnopat &  Patterns are removed from the thought. & Shawn started with 5 toys. If he got 2 toys each from his mom and dad, then that is 4 more toys.\\  \midrule
\ponlypat & Only pattern is retained in thoughts. &  5 \pathl{+} (2 \pathl{*} 2) \pathl{=} 9. \\  \midrule
\multicolumn{3}{c}{$\LHD\,$\textbf{Text}$\,\RHD$}\\\toprule
\ptextdiffentities  & Replaced with different entities of the same type (e.g. Shawn $\mapsto$ Teddy, Toys $\mapsto$ Cookies). & Teddy started with 5 cookies. If he got 2 cookies each from his Jenna and Rehan, then that is 4 more cookies. 5 + 4 = 9.\\  \midrule
\ptextrand &  Random thought from a different example is used.& Capacity of one bus is 198 passengers / 9 buses = 22 passengers in one bus. Thus, 5 buses can fit 22 * 5 = 110 passengers.    \\  \midrule
\ptextyodathought  & Only the thought is changed to be in YodaSpeak~\citep{yodaspeech}. & With 5 toys, Shawn started. 2 toys each from his mom and dad, if he got, then that is 4 more toys. 5 + 4 = 9.     \\  \midrule
\ptextintershuf &   Tokens within each sentence of a thought are shuffled.    & dad, he got 5 toys. then started mom 2 each is more that from If his and toys. toys 4 with Shawn 5 + 4 = 9.     \\  \midrule
\ptextintrashuf  &  Tokens across sentences within a thought are shuffled.      & with Shawn toys 5 started. dad, from more 2 his toys then is toys he mom got that each 4 and If. 5 + 4 = 9. \\ \bottomrule
\end{tabular}%
\caption{The summary of the counterfactual prompts used in the main text.
%
The question is ``\hltext{Shawn has five toys. For Christmas, he got two toys each from his mom and dad. How many toys does he have now?}''.
%
Unless otherwise specified, different counterfactual prompts modify different parts of both thought and questions.}
\label{tab:all_counterfactual_thoughts}
\end{table}
